The Universe at the MeV era: neutrino evolution and cosmological observables

Neutrino physics in the early Universe is key to our understanding of later cosmological stages, such as primordial nucleosynthesis (BBN) or the formation of large-scale structures. The coming decade promises new experimental results to explore and constrain cosmological models even more precisely - which requires robust theoretical predictions. This PhD thesis presents a study of the evolution of neutrinos in the first seconds after the Big Bang, more precisely when the temperature of the Universe is of the order of one mega-electronvolt. This evolution is obtained numerically by solving kinetic equations for which we propose a new derivation. A first application is the calculation of the so-called "standard" decoupling in order to calculate the cosmological parameter quantifying the energy density of the primordial relativistic species, $N_\mathrm{eff}$, to a precision of a few ten-thousandths. This study has highlighted the possibility of effectively describing the phenomenon of flavour oscillations, taking advantage of the large separation of time scales involved. Such an approximation is then adapted and validated in the case of non-zero asymmetries between neutrinos and antineutrinos. Finally, we study semi-analytically the consequences of incomplete neutrino decoupling on BBN, in order to understand how the primordial abundances of helium and deuterium are affected by this physics.

==> thcoverdata.tex <==
%!TeX encoding = UTF-8
% Metadata for coverpages
\thesisname{Thèse de doctorat}
\gradename{docteur}
\univ{de Sorbonne Université}
\logos{logo/SU.jpg}{}{logo/IAP.jpg}                   % Un à trois logo. Le 1er est celui de \univ
\specialite{Physique}
\ecoledoctnum{564}
\ecoledoct{Physique en Île-de-France}
%\title{Distorsions spectrales d'espèces relativistes en cosmologie}
%\titleen{Spectral distortions of relativistic species in cosmology}

%\title{L'Univers à l'ère du MeV : évolution des neutrinos et observables cosmologiques \\ \vspace{1em}
%\textit{\large The Universe at the MeV era: neutrino evolution and cosmological observables}}
\title{L'Univers à l'ère du MeV : évolution des neutrinos et observables cosmologiques}
\subtitle{The Universe at the MeV era: neutrino evolution and cosmological observables}
\titleen{The Universe at the MeV era: neutrino evolution and cosmological observables}

% si nécessaire, pour les métadonnées
%\titlemeta{L'Univers à l'ère du MeV : évolution des neutrinos et observables cosmologiques} 
%\titlemetaen{The Universe at the MeV era: neutrino evolution and cosmological observables} 

\date{10 juin 2022}
\author{Julien FROUSTEY}
\advisor{Cyril PITROU}
\atinstitution{à l’Institut d'Astrophysique de Paris}
\atlab{{\Large à l'Institut d'Astrophysique de Paris}}
% Jury as LaTeX Tabular. Pas de président avant soutenance								  
\jury{ %                         
M. & George FULLER & Rapporteur        \\
M. & Pasquale SERPICO  & Rapporteur       \\
M. & Marco CIRELLI & Président du jury \\
M. & Julien LESGOURGUES & Examinateur        \\
M\textsuperscript{me}& Mariam T{\'O}RTOLA & Examinatrice \\
M. & Cyril PITROU & Directeur de thèse }



\resume{La physique des neutrinos dans l'Univers primordial est un élément clé pour notre compréhension des étapes cosmologiques ultérieures, telles que la nucléosynthèse primordiale (BBN) ou la formation des grandes structures. La décennie qui s'ouvre annonce de nouveaux résultats expérimentaux permettant d'explorer et de contraindre encore plus précisément les modèles cosmologiques — ce qui nécessite des prédictions théoriques robustes. Cette thèse de doctorat présente une étude de l'évolution des neutrinos dans les premières secondes après le Big Bang, plus précisément lorsque la température de l'Univers est de l'ordre du mégaélectronvolt. Cette évolution est obtenue numériquement en résolvant des équations cinétiques dont nous proposons une nouvelle dérivation. Une première application est le calcul du découplage dit "standard" afin de calculer le paramètre cosmologique quantifiant la densité d'énergie des espèces relativistes primordiales, $N_\text{eff}$, à une précision de quelques dix-millièmes. Cette étude a mis en évidence la possibilité de décrire de manière effective le phénomène d'oscillations de saveur, en tirant profit de la large séparation d'échelles temporelles en jeu. Une telle approximation est ensuite adaptée et validée dans le cas d'asymétries non-nulles entre les neutrinos et les antineutrinos. Enfin, nous étudions semi-analytiquement les conséquences du découplage incomplet des neutrinos sur la BBN, afin de comprendre comment les abondances primordiales en hélium et deutérium sont affectées par cette physique.} %\par\hfill  (1700 car max, espaces inclus)}
\motscles{Neutrinos, cosmologie, découplage }

% si nécessaire, pour les métadonnées
%\titlemetaen{Dupondt's wool in "Land of Black Gold" } 

\abstract{ Neutrino physics in the early Universe is key to our understanding of later cosmological stages, such as primordial nucleosynthesis (BBN) or the formation of large-scale structures. The coming decade promises new experimental results to explore and constrain cosmological models even more precisely —  which requires robust theoretical predictions. This PhD thesis presents a study of the evolution of neutrinos in the first seconds after the Big Bang, more precisely when the temperature of the Universe is of the order of one mega-electronvolt. This evolution is obtained numerically by solving kinetic equations for which we propose a new derivation. A first application is the calculation of the so-called “standard” decoupling in order to calculate the cosmological parameter quantifying the energy density of the primordial relativistic species, $N_\text{eff}$, to a precision of a few ten-thousandths. This study has highlighted the possibility of effectively describing the phenomenon of flavour oscillations, taking advantage of the large separation of time scales involved. Such an approximation is then adapted and validated in the case of non-zero asymmetries between neutrinos and antineutrinos. Finally, we study semi-analytically the consequences of incomplete neutrino decoupling on BBN, in order to understand how the primordial abundances of helium and deuterium are affected by this physics.}

%\par\hfill (1700 chars max, spaces included)}
\keywords{Neutrinos, cosmology, decoupling }


